ArtMine: Discovering and Formalizing Artistic Processes

Understanding how artworks are created requires reasoning about the iterative decisions, material operations, and contextual influences that shape artistic production. While recent generative AI systems can synthesize artworks with high fidelity, they primarily model distributions over finished artifacts rather than the creative processes underlying their creation. In practice, artistic workflows are only partially documented through fragmented sources such as archival records, preparatory studies, correspondence, etc., making process-level understanding difficult to formalize computationally. In this work, we introduce ArtMine, a framework for discovering and formalizing artistic processes from heterogeneous historical evidence. Our approach synthesizes heterogeneous artwork evidence into a structured repository, from which a Peircean abductive agent infers evidence-grounded production steps. These steps are converted into a compositional graph and rendering prompt, then optimized through self-reflection over deviations between the generated and reference artworks. We provide a preliminary proof-of-concept case study using open-domain historical sources across multiple artists and artistic movements, demonstrating that fragmented documentary evidence can support coherent, interpretable, and auditable representations of artistic workflows. By modeling creative processes rather than only final artifacts, our work moves toward process-centred human-AI co-creativity systems that can support artistic interpretation, creative education, reflective collaboration, and computational studies of cultural production.

==> images/algortihm/algo.tex <==


% \newcommand\BlueCommentSty[1]{\textcolor{blue}{\scriptsize\ttfamily #1}}
% \SetCommentSty{BlueCommentSty}

\SetAlgoInsideSkip{smallskip}
\SetAlgoNlRelativeSize{-2}
\SetAlCapSkip{0.4em}

\begin{algorithm*}[t]
\scriptsize
\DontPrintSemicolon

\SetKwInOut{Input}{Input}
\SetKwInOut{Output}{Output}
\SetKwInOut{Param}{Param}

\SetKwFunction{DeepResearch}{DeepResearch}
\SetKwFunction{SeedPolicy}{SeedPolicy}
\SetKwFunction{Abduce}{Abduce}
\SetKwFunction{BuildDAG}{BuildDAG}
\SetKwFunction{BuildPrompt}{BuildPrompt}
\SetKwFunction{Strip}{StripIdentifiers}
\SetKwFunction{Render}{Render}
\SetKwFunction{Score}{Score}
\SetKwFunction{Reflect}{SelfReflect}
\SetKwFunction{Edit}{EditPolicy}
\SetKwFunction{Persist}{Persist}

\Input{Artwork sequence $A_1,\ldots,A_T$, reference images $\{I^{\mathrm{ref}}_i\}_{i=1}^{T}$,
base policy $\Pi_0$,
artwork memory $\mathcal{M}_{\mathrm{art}}$.}

\Param{iteration budget $K_{\max}$, acceptance threshold $\varepsilon_r$,
score-change threshold $\varepsilon_s$, no-progress patience $N$.}

\Output{For each artwork $A_i$: best trajectory $\tau_i^\star$,
generated image $I_i$, score vector $s_i^\star$, termination reason,
updated policy and artwork-specific memory.}

\BlankLine

$\Pi \leftarrow \Pi_0$\;

\For{$i \leftarrow 1$ \KwTo $T$}{

\tcp{\textbf{Evidence construction using DRA; see Algorithm~\ref{alg:dra-evidence}}}
$M_{\mathrm{evidence}} \leftarrow \textsc{DRA}(A_i, R_i, \mathcal{S})$\;
\tcp{DRA searches open-domain sources and fills the evidence schema field by field}
\tcp{DRA tags each claim as direct, indirect, interpretation, or speculative}
\tcp{DRA attaches sources and preserves disagreements in \texttt{conflicts}}
    \BlankLine

    \tcp{\textbf{Policy initialization}}
    $\Pi^{(0)} \leftarrow$ \SeedPolicy{$\Pi,\mathcal{M}_{\mathrm{art}}[A_i]$}\;
    $\mathcal{M}_{\mathrm{art}}\leftarrow\varnothing$;\quad
    $\mathit{best}\leftarrow\varnothing$;\quad
    $\mathit{drops}\leftarrow0$;\quad
    $\mathit{reason}\leftarrow\textsc{budget}$\;

    \BlankLine

    \For{$k \leftarrow 0$ \KwTo $K_{\max}-1$}{

        \tcp{\textbf{Abductive trajectory}}
        $\tau^{(k)} \leftarrow$ \Abduce{$\Pi^{(k)},M_{\mathrm{evidence}}$}\;
        reject any step whose observation cannot be traced to an evidence key\;

        \BlankLine

        \tcp{\textbf{Trajectory to composition DAG}}
        $G^{(k)} \leftarrow$ $\tau^{(k)}$\;
        extract visual elements and attributes from each step\;
        add edges for dependency and relative position\;
        select focal elements $v^\star$ by dependency degree and evidence support\;

        \BlankLine

        \tcp{\textbf{DAG to image-generation prompt}}
        $P^{(k)} \leftarrow$ ($G^{(k)},v^\star$) \;
        lead with the focal element and place other elements through graph relations\;
        $P^{(k)} \leftarrow$ \Strip{$P^{(k)}$}\;
        \tcp*[r]{remove artist and artwork identifiers}

        \BlankLine

        \tcp{\textbf{Render and score}}
        $I^{(k)} \leftarrow$ \Render{$P^{(k)}$}\;
        $s^{(k)} \leftarrow$ \Score{$I^{(k)},I_{\mathrm{ref}}$}\;
        \tcp*[r]{$s=(s_{\mathrm{style}},s_{\mathrm{perc}},s_{\mathrm{sem}})$}

        \If{$\mathit{best}=\varnothing$ \textbf{or} $\bar{s}^{(k)}>\bar{s}_{\mathit{best}}$}{
            $\mathit{best}\leftarrow(k,\tau^{(k)},I^{(k)},s^{(k)})$\;
        }

        \BlankLine

        \tcp{\textbf{Self-reflection}}
        $r^{(k)} \leftarrow$ \Reflect{$I^{(k)},I^{\mathrm{ref}}_i,s^{(k)},\tau^{(k)}$}\;
        extract mismatch severity $\sigma$\;
        split proposed corrections into generic principles $\mathcal{C}_g$
        and artwork-specific corrections $\mathcal{C}_a$\;

        \BlankLine

        \tcp{\textbf{Termination check}}
        $\Delta^{(k)} \leftarrow$ relative score change from $s^{(k-1)}$ to $s^{(k)}$\;

        \uIf{$\sigma < \varepsilon_r$ \textbf{and} $\max_j \Delta^{(k)}_j < \varepsilon_s$}{
            $\mathit{reason}\leftarrow\textsc{accepted}$\;
            \textbf{break}\;
        }
        \uElseIf{$k>0$ \textbf{and} $\bar{s}^{(k)} < \bar{s}^{(k-1)}$}{
            $\mathit{drops}\leftarrow\mathit{drops}+1$\;
            \If{$\mathit{drops}\ge N$}{
                $\mathit{reason}\leftarrow\textsc{no-progress}$\;
                \textbf{break}\;
            }
        }
        \Else{
            $\mathit{drops}\leftarrow0$\;
        }

        \BlankLine

        \tcp{\textbf{Policy update}}
        \eIf{$\sigma \ge \varepsilon_r$}{
            add non-duplicate $\mathcal{C}_g$ to the generic policy principles\;
            add $\mathcal{C}_a$ to $\mathcal{M}_{\mathrm{art}}[A_i]$ as worked examples\;
            $\Pi^{(k+1)} \leftarrow$ \Edit{$\Pi^{(k)},r^{(k)}$}\;
        }{
            $\Pi^{(k+1)} \leftarrow \Pi^{(k)}$\;
        }
    }

    \BlankLine

      $(k^\star,\tau_i^\star,\hat I_i,s_i^\star)\leftarrow\mathit{best}$\;

    \tcp{\textbf{Persist learned state}}
    $\Pi^{(k^\star)} \leftarrow (R,\Sigma \cup \mathcal{C}_{g}, C \cup \mathcal{C}_{a})$\;
    \Persist{$\mathcal{M}_{\mathrm{art}}[A_i]$ with artwork-specific corrections}\;

}

\Return $\{(\tau_i^\star,\hat I_i,s_i^\star,\mathit{reason}_i)\}_{i=1}^{T}$,
$\Pi$, $\mathcal{M}_{\mathrm{art}}$\;

\caption{Abductive reconstruction and cross-artwork policy transfer.}
\label{alg:full-method}
\end{algorithm*}




==> images/algortihm/dra.tex <==
\newcommand\BlueCommentSty[1]{\textcolor{blue}{\scriptsize\ttfamily #1}}
\SetCommentSty{BlueCommentSty}

\SetAlgoInsideSkip{smallskip}
\SetAlgoNlRelativeSize{-2}
\SetAlCapSkip{0.4em}

\begin{algorithm}[t]
\scriptsize
\DontPrintSemicolon

\SetKwInOut{Input}{Input}
\SetKwInOut{Output}{Output}
\SetKwInOut{Param}{Param}

\SetKwFunction{Search}{SearchWeb}
\SetKwFunction{Retrieve}{RetrieveSources}
\SetKwFunction{Extract}{ExtractClaims}
\SetKwFunction{Classify}{ClassifyEvidence}
\SetKwFunction{Conflict}{DetectConflicts}
\SetKwFunction{Store}{StoreClaim}

\Input{Artwork name $A$, artist name $R$, predefined evidence schema $\mathcal{S}$.}

\Param{Source types $\mathcal{T}=\{$museum records, catalogues, artist correspondence,
conservation reports, technical studies, provenance records, scholarly sources$\}$.}

\Output{Structured evidence repository $M_{\mathrm{evidence}}$.}

\BlankLine

$M_{\mathrm{evidence}} \leftarrow \mathcal{S}$\;
$M_{\mathrm{evidence}}[\texttt{conflicts}] \leftarrow \emptyset$\;
$\mathcal{D} \leftarrow \emptyset$\;

\BlankLine

\tcp{\textbf{Source discovery}}
$\mathcal{Q} \leftarrow$ build search queries from artwork name $A$, artist name $R$, and schema fields in $\mathcal{S}$\;

\ForEach{source type $t \in \mathcal{T}$}{
    $\mathcal{D}_t \leftarrow$ \Search{$A,R,t,\mathcal{Q}$}\;
    $\mathcal{D} \leftarrow \mathcal{D} \cup \mathcal{D}_t$\;
}

\BlankLine

\tcp{\textbf{Schema-guided extraction}}
\ForEach{schema field $s \in \mathcal{S}$}{

    $\mathcal{K}_s \leftarrow \emptyset$\;
    
    \ForEach{source document $d \in \mathcal{D}$}{
        $\mathcal{C} \leftarrow$ \Extract{$d,s$}\;
        
        \ForEach{claim $c \in \mathcal{C}$}{
            $\tau \leftarrow$ \Classify{$c,d$}\;
            \tcp*[r]{$\tau \in \{\textsc{Direct},\textsc{Indirect},\textsc{Interpretation},\textsc{Speculative}\}$}
            
            attach source reference $\mathrm{src}(c)\leftarrow d$\;
            $\mathcal{K}_s \leftarrow \mathcal{K}_s \cup \{(c,\mathrm{src}(c),\tau)\}$\;
        }
    }

    \BlankLine

    \eIf{$\mathcal{K}_s=\emptyset$}{
        $M_{\mathrm{evidence}}[s]\leftarrow \textsc{Unknown}$\;
    }{
        $(\mathcal{K}^{+}_s,\mathcal{K}^{\mathrm{conf}}_s) \leftarrow$ \Conflict{$\mathcal{K}_s$}\;
        \ForEach{$(c,\mathrm{src}(c),\tau)\in \mathcal{K}^{+}_s$}{
            \Store{$M_{\mathrm{evidence}}[s],c,\mathrm{src}(c),\tau$}\;
        }
        \If{$\mathcal{K}^{\mathrm{conf}}_s \neq \emptyset$}{
            $M_{\mathrm{evidence}}[\texttt{conflicts}][s]\leftarrow \mathcal{K}^{\mathrm{conf}}_s$\;
        }
    }
}

\BlankLine

\tcp{\textbf{Repository finalization}}
verify every non-unknown claim has a source reference and evidence type\;
preserve unknown fields and conflicting claims without merging them\;

\Return $M_{\mathrm{evidence}}$\;

\caption{Deep Research Agent for evidence repository construction.}
\label{alg:dra-evidence}
\end{algorithm}
